VCR-GauS: View Consistent Depth-Normal Regularizer for Gaussian Surface Reconstruction

Although 3D Gaussian Splatting has been widely studied because of its realistic and efficient novel-view synthesis, it is still challenging to extract a high-quality surface from the point-based representation. Previous works improve the surface by incorporating geometric priors from the off-the-shelf normal estimator. However, there are two main limitations: 1) Supervising normals rendered from 3D Gaussians effectively updates the rotation parameter but is less effective for other geometric parameters; 2) The inconsistency of predicted normal maps across multiple views may lead to severe reconstruction artifacts. In this paper, we propose a Depth-Normal regularizer that directly couples normal with other geometric parameters, leading to full updates of the geometric parameters from normal regularization. We further propose a confidence term to mitigate inconsistencies of normal predictions across multiple views. Moreover, we also introduce a densification and splitting strategy to regularize the size and distribution of 3D Gaussians for more accurate surface modeling. Compared with Gaussian-based baselines, experiments show that our approach obtains better reconstruction quality and maintains competitive appearance quality at faster training speed and 100+ FPS rendering.

==> tables/replica_ablation.tex <==
% \begin{table}[htbp]
%     \centering
%     \small
%     \caption{\textbf{Ablation on TNT Dataset.}}
%     \begin{tabular}{l|ccc}
%     \hline
%      & Precision~$\uparrow$ & Recall~$\uparrow$ & F-score \\
%     \hline
%     A. w/o d-normal & 0.27 & 0.34 & 0.30 \\
%     B. w/o confidence & 0.36 & 0.37 & 0.36 \\
%     C. w/o intersection depth & 0.35 & 0.37 & 0.35 \\
%     D. w/o densify and split & 0.32 & 0.35 & 0.33 \\
%     \hline
%     E. Full & 0.39 & 0.42 & 0.40 \\
%     \hline
%     \end{tabular}
%         \label{tab:tnt_ablation}
% \end{table}

\begin{table}[h]
    \small
    \centering
    \label{tab:combined}
    \begin{minipage}{0.38\textwidth}
        \setlength\tabcolsep{1pt}
        \renewcommand\arraystretch{0.7}
        \centering
        \small
        \caption{\small 
             \textbf{Quantitative assessment on Replica \cite{straub2019replica}}. \textbf{Bold} indicates best result.
            }
        \label{tab:replica}
        % \resizebox{1\textwidth}{!}{
        \begin{tabular}{c|c|c|c}
        % \begin{tabular}{cccc}
        \toprule
        & Method & F1-score & Time \\
        \midrule
        \multirow{2}{*}{Implicit} & NeuS & 65.12 & >10 h \\
        & MonoSDF & \textbf{81.64} & \\
        \midrule
        \multirow{4}{*}{Explicit} & 3DGS & 50.79 & \multirow{4}{*}{<= 1 h} \\
        & SuGar & 63.20 & \\
        & 2DGS & 64.36 & \\
        & Ours & \textbf{78.12} & \\
        \toprule
        \end{tabular}
        % }
    \end{minipage}
    \hfill
    \begin{minipage}{0.6\textwidth}
        % \renewcommand\arraystretch{1.3}
        \centering
        \caption{\textbf{Ablation on TNT~\cite{knapitsch2017tanks}.} \textbf{Bold} indicates best result.}
        \label{tab:tnt_ablation}
        % \begin{tabular}{l|ccc}
        \begin{tabular}{lccc}
        \toprule
         & Precision~$\uparrow$ & Recall~$\uparrow$ & F-score \\
        \hline
        A. w/o d-normal & 0.27 & 0.34 & 0.30 \\
        B. w/o confidence & 0.36 & 0.37 & 0.36 \\
        C. w/o intersection depth & 0.35 & 0.37 & 0.35 \\
        D. w/o densify and split & 0.32 & 0.35 & 0.33 \\
        \hline
        E. Full & 0.39 & 0.42 & \textbf{0.40} \\
        \toprule
        \end{tabular}
    \end{minipage}
\end{table}

